Unraveling the Impact of Visual Complexity on Search as Learning

Information search has become essential for learning and knowledge acquisition, offering broad access to information and learning resources. The visual complexity of web pages is known to influence search behavior, with previous work suggesting that searchers make evaluative judgments within the first second on a page. However, there is a significant gap in our understanding of how visual complexity impacts searches specifically conducted with a learning intent. This gap is particularly relevant for the development of optimized information retrieval (IR) systems that effectively support educational objectives. To address this research need, we model visual complexity and aesthetics via a diverse set of features, investigating their relationship with search behavior during learning-oriented web sessions. Our study utilizes a publicly available dataset from a lab study where participants learned about thunderstorm formation. Our findings reveal that while content relevance is the most significant predictor for knowledge gain, sessions with less visually complex pages are associated with higher learning success. This observation applies to features associated with the layout of web pages rather than to simpler features (e.g., number of images). The reported results shed light on the impact of visual complexity on learning-oriented searches, informing the design of more effective IR systems for educational contexts. To foster reproducibility, we release our source code (https://github.com/TIBHannover/sal_visual_complexity).

==> tables/all_features_description.tex <==
\begin{table}[htb]
\setlength{\tabcolsep}{2.9pt}
\centering
\fontsize{9}{10}\selectfont
\def\arraystretch{0.4}
\caption{Name, description, and origin of the visual complexity features}
\label{tab:all_features_description}
\begin{tabular}{lcllc}
\toprule
 &  & \textbf{Name} & \textbf{Description} & \textbf{Origin} \\
\midrule
\multirow{20}{*}{\rotatebox[origin=c]{90}{\textbf{HTML}}} & \texttt{f1} & \texttt{n\_text\_obj} & Number of text objects & \cite{Wu13Measuring} \\
 & \texttt{f2} & \texttt{n\_link\_obj} & Number of link objects & \cite{Wu13Measuring,Yu2021} \\
 & \texttt{f3} & \texttt{n\_par\_obj} & Number of paragraphs & \cite{Wan21novel} \\
 & \texttt{f4} & \texttt{n\_img\_obj} & Number of image objects & \cite{Wan21novel,Yu2021} \\
 & \texttt{f5} & \texttt{n\_form\_obj} & Number of form objects & \cite{Wan21novel} \\
 & \texttt{f6} & \texttt{n\_list\_obj} & Number of list objects & \cite{Wan21novel} \\
 & \texttt{f7} & \texttt{n\_table\_obj} & Number of table objects & \cite{Wu13Measuring} \\
 & \texttt{f8} & \texttt{max\_words\_par} & Number of words in the longest paragraph & \cite{Wan21novel} \\
 & \texttt{f9} & \texttt{min\_words\_par} & Number of words in the shortest paragraph & \cite{Wan21novel} \\
 & \texttt{f10} & \texttt{avg\_word\_par} & Average number of words per paragraph & \cite{Wan21novel,Yu2021} \\
 & \texttt{f11} & \texttt{std\_div\_words\_par} & Standard dev. of words per paragraph & \cite{Wan21novel} \\
 & \texttt{f12} & \texttt{n\_links\_per\_par} & Number of links per paragraph & \cite{Wu13Measuring} \\
 & \texttt{f13} & \texttt{n\_headl\_per\_par} & Number of headlines per paragraph & ours \\
 & \texttt{f14} & \texttt{headl\_depth} & Headline depth (’h1’ to ’h6’ equals depth of 6) & ours \\
 & \texttt{f15} & \texttt{n\_fonts} & Number of fonts & \cite{Wu13Measuring} \\
 & \texttt{f16} & \texttt{n\_font\_sizes} & Number of font sizes & \cite{Wu13Measuring} \\
 & \texttt{f17} & \texttt{avg\_font\_size} & Average font size & \cite{Wu13Measuring} \\
 & \texttt{f18} & \texttt{n\_font\_weights} & Number of font weights & \cite{Wu13Measuring} \\
 & \texttt{f19} & \texttt{avg\_font\_weight} & Average font weight & \cite{Wu13Measuring} \\
 & \texttt{f20} & \texttt{n\_bg\_colors} & Number of background colors & \cite{Wu13Measuring} \\
\midrule
\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Visual}}} & \texttt{f21} & \texttt{avg\_brightness} & Average brightness & \cite{Wu13Measuring} \\
 & \texttt{f22} & \texttt{avg\_hue} & Average hue & \cite{Wu13Measuring} \\
 & \texttt{f23} & \texttt{avg\_colorfulness} & Average colorfulness & \cite{Wu13Measuring} \\
 & \texttt{f24 - f25} & \texttt{png\_size / jpg} & PNG size / JPG size & \cite{Wu13Measuring} \\
 & \texttt{f26 - f27} & \texttt{norm\_png\_size / jpg} & Normalized PNG / JPG size & \cite{Wu13Measuring} \\
 & \texttt{f28} & \texttt{page\_width\_page\_height} & Page’s $width + height$ & \cite{Wu13Measuring} \\
 & \texttt{f29} & \texttt{aspect\_ratio} & Aspect ratio (page’s $\frac{height}{width}$) & \cite{Wu13Measuring} \\
\midrule
\multirow{15}{*}{\rotatebox[origin=c]{90}{\textbf{Layout}}} & \texttt{f30} & \texttt{n\_vips\_non\_leaf\_nodes} & Number of non-leaf nodes & \cite{Wu13Measuring} \\
 & \texttt{f31} & \texttt{n\_vips\_leaf\_nodes} & Number of leaf nodes & \cite{Wu13Measuring} \\
 & \texttt{f32} & \texttt{n\_vips\_nodes\_two\_child} & Number of nodes with two children & \cite{Wu13Measuring} \\
 & \texttt{f33} & \texttt{n\_vips\_nodes\_three\_child} & Number of nodes with three children & \cite{Wu13Measuring} \\
 & \texttt{f34} & \texttt{n\_vips\_nodes\_four\_child} & Number of nodes with four children & \cite{Wu13Measuring} \\
 & \texttt{f35} & \texttt{n\_vips\_nodes\_five\_child} & Number of nodes with five children & \cite{Wu13Measuring} \\
 & \texttt{f36} & \texttt{n\_vips\_nodes\_more\_child} & Number of nodes with more than five children & \cite{Wu13Measuring} \\
 & \texttt{f37} & \texttt{n\_vips\_text\_nodes} & Number of text nodes & ours \\
 & \texttt{f38} & \texttt{n\_vips\_text\_leaf\_nodes} & Number of text leaf nodes & \cite{Wu13Measuring} \\
 & \texttt{f39} & \texttt{n\_texts\_to\_whole\_page} & Number of texts in proportion to whole page & \cite{Wu13Measuring} \\
 & \texttt{f40} & \texttt{text\_area\_to\_whole\_page} & Total text area in proportion to whole page & \cite{Wu13Measuring} \\
 & \texttt{f41} & \texttt{n\_texts\_to\_text\_area} & Number of texts to total text area & \cite{Wu13Measuring} \\
 & \texttt{f42} & \texttt{n\_vips\_img\_nodes} & Number of images nodes & ours \\
 & \texttt{f43} & \texttt{n\_vips\_img\_leaf\_nodes} & Number of images leaf nodes & ours \\
 & \texttt{f44} & \texttt{n\_vips\_layers} & Number of layers & \cite{Wu13Measuring} \\
\midrule
\multirow{18}{*}{\rotatebox[origin=c]{90}{\textbf{Aesthetic}}} & \texttt{f45} & \texttt{balance} & Balance & \cite{Ling2003Modelling,Wan21novel} \\
 & \texttt{f46} & \texttt{equilibrium} & Equilibrium & \cite{Ling2003Modelling,Wan21novel} \\
 & \texttt{f47} & \texttt{symmetry} & Symmetry & \cite{Ling2003Modelling,Wan21novel} \\
 & \texttt{f48} & \texttt{sequence} & Sequence & \cite{Ling2003Modelling,Wan21novel} \\
 & \texttt{f49} & \texttt{cohesion} & Cohesion & \cite{Ling2003Modelling,Wan21novel} \\
 & \texttt{f50} & \texttt{unity} & Unity & \cite{Ling2003Modelling,Wan21novel} \\
 & \texttt{f51} & \texttt{proportion} & Proportion & \cite{Ling2003Modelling,Wan21novel} \\
 & \texttt{f52} & \texttt{simplicity} & Simplicity & \cite{Ling2003Modelling,Wan21novel} \\
 & \texttt{f53} & \texttt{density} & Density & \cite{Ling2003Modelling,Wan21novel} \\
 & \texttt{f54} & \texttt{regularity} & Regularity & \cite{Ling2003Modelling,Wan21novel} \\
 & \texttt{f55} & \texttt{economy} & Economy & \cite{Ling2003Modelling,Wan21novel} \\
 & \texttt{f56} & \texttt{homogeneity} & Homogeneity & \cite{Ling2003Modelling,Wan21novel} \\
 & \texttt{f57} & \texttt{rhythm} & Rhythm & \cite{Ling2003Modelling,Wan21novel} \\
 & \texttt{f58} & \texttt{order\_and\_complexity} & Order and Complexity & \cite{Ling2003Modelling,Wan21novel} \\
 & \texttt{f59 - f72} &  & Same features text-based & \cite{Wan21novel} \\
 & \texttt{f73 - f86} &  & Same features image-based & \cite{Wan21novel} \\
 & \texttt{f87 - f100} &  & Same features form-based & \cite{Wan21novel} \\
 & \texttt{f101 - f114} &  & Same features other-based & \cite{Wan21novel} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/html_tags_groupings_overview.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{2.0pt}
\centering
\fontsize{8}{10}\selectfont
\def\arraystretch{0.8}
\caption{Overview of HTML Tags and their groupings}
\label{tab:html-tags}
\begin{tabular}{lp{0.75\linewidth}}
\toprule
\textbf{Tag Group} & \textbf{HTML Tags} \\
\midrule
\textit{Links} & \texttt{<a>} \\
\textit{Paragraphs} & \texttt{<p>} \\
\textit{Headings} & \texttt{<h1>, <h2>, <h3>, <h4>, <h5>, <h6>} \\
\textit{Text Elements} & \texttt{<b>, <i>, <u>, <s>, <code>, <cite>, <em>, <strong>, <abbr>, <acronym>, <address>, <bdo>, <blockquote>, <q>, <ins>, <dfn>, <kbd>, <pre>, <samp>, <var>, <br>, <del>} \\
\textit{Images} & \texttt{<img>, <canvas>, <video>, <map>, <area>} \\
\textit{Forms} & \texttt{<button>, <input>, <textarea>, <select>, <output>, <form>, <keygen>, <option>, <optgroup>, <label>, <fieldset>, <legend>} \\
\textit{Lists} & \texttt{<ul>, <ol>, <li>, <dl>, <dt>, <dd>} \\
\textit{Tables} & \texttt{<table>, <tr>, <td>, <th>, <tbody>, <thead>, <tfoot>, <col>, <colgroup>, <caption>} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/top12_selected_features_correlation_with_kg.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{2.9pt}
\centering
\fontsize{9}{10}\selectfont
%\def\arraystretch{1.5}
\caption{Correlation between the top 10 visual complexity features and the knowledge gain}
\label{tab:top12_correlation}
\begin{tabular}{lccc}
\toprule
\textbf{Feature Name} & \textbf{Pearson r} & \textbf{p} & \textbf{$\text{p}_\text{FDR}$} \\
\midrule
\textbf{Links per Paragraph} & \textbf{-0.230} & \textbf{0.015} & \textbf{0.018} \\
\textbf{Form Order and Complexity} & \textbf{-0.222} & \textbf{0.020} & \textbf{0.022} \\
\textbf{Text Rhythm} & \textbf{-0.246} & \textbf{0.010} & \textbf{0.015} \\
\textbf{Other Order and Complexity} & \textbf{-0.251} & \textbf{0.009} & \textbf{0.015} \\
\textbf{Image Cohesion} & \textbf{-0.298} & \textbf{0.002} & \textbf{0.015} \\
\textbf{Form Regularity} & \textbf{-0.257} & \textbf{0.007} & \textbf{0.015} \\
\textbf{Rhythm} & \textbf{-0.264} & \textbf{0.005} & \textbf{0.015} \\
Texts in proportion to whole page & -0.181 & 0.056 & 0.056 \\
\textbf{Text Proportion} & \textbf{-0.236} & \textbf{0.013} & \textbf{0.018} \\
\textbf{Other Rhythm} & \textbf{-0.266} & \textbf{0.005} & \textbf{0.015} \\
\textbf{Other Symmetry} & \textbf{-0.251} & \textbf{0.008} & \textbf{0.015} \\
\textbf{Form Simplicity} & \textbf{-0.251} & \textbf{0.009} & \textbf{0.015} \\
\bottomrule
\end{tabular}
\end{table}
